CHARD: Clinical Health-Aware Reasoning Across Dimensions for Text Generation Models

We motivate and introduce CHARD: Clinical Health-Aware Reasoning across Dimensions, to investigate the capability of text generation models to act as implicit clinical knowledge bases and generate free-flow textual explanations about various health-related conditions across several dimensions. We collect and present an associated dataset, CHARDat, consisting of explanations about 52 health conditions across three clinical dimensions. We conduct extensive experiments using BART and T5 along with data augmentation, and perform automatic, human, and qualitative analyses. We show that while our models can perform decently, CHARD is very challenging with strong potential for further exploration.

==> sections/TODO.tex <==
-IAA for human eval
-Final human eval stat sig (bootstrap)
-First-page model diagram



COMPLETED:

-Task (DONE)
    -Come up with name for our task (DONE)
    -Brief description with examples and purpose (DONE)
    -Describe dimensions (DONE)
    -Discuss the task formulation: template infilling (DONE)
-Dataset (DONE)
    -Come up with name for our dataset (DONE)
    -Collection process (including AMT details) (DONE - NEED MORE IN APPENDIX)
    -Qual examples of dataset writings (by dimension) (DONE - NEED MORE IN APPENDIX)
    -Train, val, test splits (DONE)
        -Test split half seen, half unseen (DONE)
    -Stats (table - total and broken down by dimension, per split) (DONE)
        -Include average length (in words) (DONE)

-Methodology (DONE)
    -Models (BART, T5, two sizes) (DONE)
    -Backtranslation data aug
        -Describe UDA backtranslation (DONE)
        -Temperatures (DONE)
        -Qual examples of backtranslations by temp (DONE)
        -Backtranslation analysis (BERTScore vs. ROUGE by temp) - graphs and tables (DONE)
    -Automatic eval metrics (DONE)
-Experimental setup: (DONE)
    -Model finetuning + generation details (DONE)
    -Also individual dimensions vs. combined models (DONE)
    -Backtranslation data aug details (DONE)
        -E.g. try all temperatures on 2x and various data aug amounts (and best vs. diff temps) on base models, then try top temps (and only 3x, 5x, 7x, 10x with either best or diff temps) with large models (DONE)
    -Human eval details (models, # of examples, eval dimensions, pairwise setup) (DONE)

-Combined model results per individual dimension (DONE)
-Finalize title of the paper (DONE)

-Results and Analysis
    -Tables and graphs
        -Table with retrieval, best of BART-base, T5-base, BART-large, and T5-large (note down human length and PPL in the caption) (DONE)
        -Table with T5-large broken down into seen and unseen test splits (DONE)
        -Graphs of x2 model ROUGE-2 values by backtranslation temps (DONE)
        -Graphs of model ROUGE-2 values by data aug amount (DONE)
        -Table with T5-large broken down into individual dimension models (DONE)
        -Human eval table with averages by eval aspect (T5 vs. human, retrieval vs. human, retrieval vs. T5) (NEED TO FILL IN)
            -Include stat sig and maybe IAA values in the table (NEED TO FILL IN)
        -Qual example table with human, retrieval, best BART-large, T5-large (maybe BART-base, T5-base) (DONE)
            -Mix of seen and unseen test examples (DONE)
            -Mix of examples per dimension (prevention, treatment, risk factor) (DONE)
            -Examples where our models do better than retrieval and where we do worse (DONE)
    -Automatic results analysis (DONE)
        -Analysis of overall results, individual dimension vs. combined model, seen vs. unseen test splits (DONE)
        -Analysis of data aug: backtrans temp + data aug amount (DONE)
    -Human results analysis (NEED RESULTS)
        -Analysis of overall results
    -Qualitative analysis (DONE)
        -Discuss where our models differ from humans and retrieval (both better and worse) (DONE)
        -Discuss how our models perform per dimension and test split half (DONE)
        -Discuss T5 vs. BART and large vs. base models (DONE)

-Human eval average scores (using scores so far) (DONE)
-Human eval results table + analysis (using scores so far) (DONE)

-Takeways & directions for improvement (DONE)
-Future work (DONE)
-Conclusion (DONE)
-Abstract (DONE)

-Related work (Dheeraj paper, other papers Vivek sent, then find some others) (DONE)
    -Template infilling work (e.g. STE, Mina and Percy's paper, Dheeraj paper)
    -Commonsense reasoning (e.g. COMET, CommonGen, SAPPHIRE, Yejin Choi's work, etc.)
    -Retrieval and extraction-based healthcare reasoning work (e.g. papers and links that Vivek emailed to me)
-Intro (good story + contributions) (DONE)

-Cut paper down to 8 pages body (DONE)
-Appendices (IGNORE)
    -Additional examples from our dataset (FORGET IT) 
    -Additional human eval results broken down by dimension (FORGET IT)
    -Additional backtranslation data aug details (NOT UNNECESSARY)
    -Additional val split result graphs and/or tables (e.g. ROUGE-2) by backtranslation temp, amount, best temp vs. diff temps, model, etc. (NOT NECESSARY)
-Final human eval average scores (DONE)
-Changes to human eval explanation, results, and analysis (DONE)
-Ethics statement (look at Diyi Yang, Dheeraj paper, and my past papers) (DONE)
    -no personal/private info, general clinical info
    -not used in real-world use-case, simply for investigation purposes (write clearly: hypothesis and based on results, we can clearly see that it should not be used for any diagnosis yet) - look at dheeraj paper for similar statement
    -pay for eval: \$0.2 per hit, overall pay was higher than \$X, higher than min wage (look at Dheeraj paper)
-Appendices (DONE)
    -Additional human eval details (including template screenshots or say it's in the supplementary .zip files) (DONE)
    -Additional human annotation details (including template screenshots or say it's in the supplementary .zip files) (DONE)
    -Full list of conditions (52) (DONE)
    -Further qualitative examples (maybe for more models, e.g. individual dim models for T5-large, diff data aug models by temp and amount) (DONE)
    -Additional model finetuning + generation details (DONE)
-Submit on the portal (add all authors, etc.) (DONE)
-Clean up code and data (into .zip files) and submit them (DONE)
-Print out and go through things one final time (DONE)
-Ensure everything is good: style, formatting, page limits, references, follows submission guidelines, and submission info all good (DONE)
